Dynamic Pattern Matching with Wildcards

We study the fully dynamic pattern matching problem where the pattern may contain up to kwildcard symbols, each matching any symbol of the alphabet. Both the text and the pattern are subject to updates (insert, delete, change). We design an algorithm with O(nlog^2 n) preprocessing and update/query time O(knk/k+1 + k2 log n). The bound is truly sublinear for a constant k, and sublinear when k= o(log n). We further complement our results with a conditional lower bound: assuming subquadratic preprocessing time, achieving truly sublinear update time for the case k = {\Omega}(log n) would contradict the Strong Exponential Time Hypothesis (SETH). Finally, we develop sublinear algorithms for two special cases: - If the pattern contains w non-wildcard symbols, we give an algorithm with preprocessing time O(nw) and update time O(w + log n), which is truly sublinear whenever wis truly sublinear. - Using FFT technique combined with block decomposition, we design a deterministic truly sublinear algorithm with preprocessing time O(n^1.8) and update time O(n^0.8 log n) for the case that there are at most two non-wildcards.

==> src/dynamic-wildcard-at-most-two.tex <==
% Ops
\newcommand{\get}[5]{\texttt{get}(#1,#2,#3,#4,#5)}
\newcommand{\change}[2]{\texttt{change}(#1,#2)}




==> src/hash-queries-segment-tree-pseudocode.tex <==
\begin{document}

\begin{algorithm}
\caption{Segment Tree for Hash Queries on String \(S\)}
\begin{algorithmic}[1]
\State \textbf{Input:} String \(S \in \alphabet^*\) of length \(|S|\), modulus \(p\), base \(\text{base}\)
\State \textbf{Global:} Array \(\text{powers}[k] = \text{base}^{k} \mod p\) for \(k = 0\) to \(|S|\)
\State \textbf{Data Structure:} Segment tree where node \(v\) stores \(\hashFunc{S_{\ell_v:r_v}}\) for interval \([\ell_v, r_v]\)

\Function{PrecomputePowers}{$|S|, p, \text{base}$}
    \State \textbf{Output:} Array \(\text{powers}[0 \dots |S|]\)
    \State \(\text{powers}[0] \gets 1\)
    \For{\(k \gets 1\) to \(|S|\)}
        \State \(\text{powers}[k] \gets (\text{powers}[k-1] \cdot \text{base}) \mod p\) \Comment{\(\BigONotation(d \log d)\) per multiplication}
    \EndFor \Comment{Total: \(\BigONotation(|S| \cdot d \log d)\)}
    \State \Return \(\text{powers}\)
\EndFunction

\Function{MergeNodes}{$h_{\text{left}}, h_{\text{right}}, \text{len}_{\text{right}}$}
    \State \textbf{Input:} Left hash \(h_{\text{left}} = \hash(S[\ell, m])\), right hash \(h_{\text{right}} = \hash(S[m+1, r])\), right length \(\text{len}_{\text{right}} = r - m\)
    \State \textbf{Output:} Combined hash \(\hash(S[\ell, r])\)
    \State \Return \(\left( h_{\text{left}} \cdot \text{powers}[\text{len}_{\text{right}}] + h_{\text{right}} \right) \mod p\)
    \Comment{\(\BigONotation(d \log d)\) per concatenation}
\EndFunction

\Function{BuildSegmentTree}{$S, p, \text{base}$}
    \State \textbf{Initialize powers:}
    \State \(\text{powers} \gets \text{PrecomputePowers}(|S|, p, \text{base})\)
    \State \textbf{Construct tree:}
    \State Initialize segment tree with \(|S|\) leaves
    \For{each leaf node \(v\) at position \(i\)}
        \State \(\hash(S[i, i]) \gets S[i] \mod p\) \Comment{Leaf hash, \(\BigONotation(1)\)}
    \EndFor
    \For{each internal node \(v\) with children \(v_{\text{left}}, v_{\text{right}}\) covering \([\ell_v, m], [m+1, r_v]\)}
        \State \(\hash(S[\ell_v, r_v]) \gets \text{MergeNodes}(\hash(S[\ell_v, m]), \hash(S[m+1, r_v]), r_v - m)\)
    \EndFor \Comment{Total: \(\BigONotation(|S| \cdot d \log d)\)}
\EndFunction

\Function{RangeQuery}{$S, \ell, r$}
    \State \textbf{Output:} \(\hash(S[\ell, r])\)
    \State Initialize empty list \(L\) of intervals
    \State Decompose \([\ell, r]\) into \(\BigONotation(\log |S|)\) canonical intervals using segment tree
    \For{each canonical interval \([\ell_i, r_i]\) in \(L\)}
        \State Retrieve \(\hash(S[\ell_i, r_i])\) from node covering \([\ell_i, r_i]\)
    \EndFor
    \State Initialize \(\text{result} \gets 0\)
    \For{each interval \([\ell_i, r_i]\) in \(L\) from left to right}
        \State \(\text{result} \gets \text{MergeNodes}(\text{result}, \hash(S[\ell_i, r_i]), r_i - \ell_i + 1)\)
    \EndFor
    \State \Return \(\text{result}\)
    \Comment{Total: \(\BigONotation(\log |S| \cdot d \log d)\)}
\EndFunction

\Function{UpdateQuery}{$S, i, c$}
    \State \textbf{Input:} Position \(i\), new symbol \(c \in \alphabet\)
    \State Update \(S[i] \gets c\)
    \State Identify \(\BigONotation(\log |S|)\) nodes whose intervals \([\ell_v, r_v]\) contain position \(i\)
    \For{each node \(v\) with interval \([\ell_v, r_v]\)}
        \If{\(\ell_v = r_v = i\)} \Comment{Leaf node}
            \State \(\hash(S[i, i]) \gets c \mod p\) \Comment{\(\BigONotation(1)\)}
        \Else \Comment{Internal node}
            \State Let \(v_{\text{left}}, v_{\text{right}}\) cover \([\ell_v, m], [m+1, r_v]\)
            \If{\(i \leq m\)}
                \State Recursively update left child \(v_{\text{left}}\)
            \Else
                \State Recursively update right child \(v_{\text{right}}\)
            \EndIf
            \State \(\hash(S[\ell_v, r_v]) \gets \text{MergeNodes}(\hash(S[\ell_v, m]), \hash(S[m+1, r_v]), r_v - m)\)
        \EndIf
    \EndFor
    \Comment{Total: \(\BigONotation(\log |S| \cdot d \log d)\)}
\EndFunction

\end{algorithmic}
\end{algorithm}

\end{document}

==> src/matchingwithnochangeinT.tex <==
\textbf{Matching in Unmodified Segments of \(\textstr\):}  
In this case we exploit the modified hash function \(\hashPrimeFunc{\cdot}\) together with the precomputed array \(A\).  
If a candidate substring \(\textstr_{\ell : \ell + \lengthP - 1}\) lies entirely within a region of the text that
has not been altered since preprocessing, its hash value \(\hashPrimeFunc{\textstr_{\ell : \ell + \lengthP - 1}}\) remains valid. 
To check for a match, we simply test whether the pattern hash \(\hashPrimeFunc{\pattern}\) appears among the precomputed values in
the relevant portion of \(A\):  
\[
\exist\big(A_{\ell : r - \lengthP + 1}, \, \hashPrimeFunc{\pattern}\big).
\]

Since we rebuild all data structures every \(\tau\) updates, the number of modifications that may have occurred since 
the most recent preprocessing step is at most \(\tau\). These modifications divide \(\textstr\) into at most 
\(\tau+1\) maximal unmodified segments.  

For each such unmodified segment \([l,r]\), we perform the existence query
\[
\exist\big(A_{l : r - \lengthP + 1}, \, \hashPrimeFunc{\pattern}\big),
\]
which checks whether any substring starting in that segment matches the pattern under \(\hashPrimeFunc{\cdot}\). Each query can be answered 
in \(\BigONotation(\log \lengthT)\) time. Since there are at most \(\tau+1 = \BigONotation(\tau)\) unmodified segments, the overall cost is
$
\BigONotation(\tau \cdot \log \lengthT).
$


==> src/nowildmatchtosmallcharacter.tex <==
\noindent\textbf{No wildcard matches a rare symbol.}  
Recall that Case~(i) already covered the situation where \(\pattern\) itself contains a rare symbol. 
Therefore, in the present case we may assume that \(\pattern\) is composed only of frequent symbols and wildcards.  

If a match exists under these conditions, then every wildcard in \(\pattern\) must align with a frequent symbol in 
\(\textstr\). To check this possibility, we explicitly test all candidate strings obtained by replacing the wildcards of 
\(\pattern\) with frequent symbols. Each such candidate is a concrete string with no wildcards, and we can check whether 
it matches some substring of \(\textstr\) by using the fully dynamic LCS data structure from Theorem~\ref{thm:lcs_query}, 
which supports single-symbol updates in \(\BigONotation(\log^8 \lengthT)\) time.  

Let the set of frequent symbols be \(F\), with \(|F| \leq \tfrac{\lengthT}{\tau}\). 
Every wildcard position in \(\pattern\) can be replaced with any symbol from \(F\).  
Thus the total number of candidate strings is bounded by
$
\left(\tfrac{\lengthT}{\tau}\right)^k.
$


To test all of them efficiently, we must generate the candidates in such a way that each consecutive string differs from 
the previous one at exactly one wildcard position. This can be achieved by enumerating the \(k\)-dimensional grid 
\([|F|]^k\) (each coordinate representing the choice of symbol for one wildcard) in a Gray-code order. Such an ordering 
ensures that two consecutive vectors differ in exactly one coordinate.  

Concretely, we map each candidate string to a vector 
\((f_1, f_2, \ldots, f_k)\), where \(f_j \in F\) specifies the substitution chosen for the \(j\)-th wildcard.  
We then enumerate all vectors of this form using a recursive construction of generalized Gray codes \cite{knuth2013art}:  

\begin{itemize}
	\item \textbf{Base case (\(k=1\)).}  
	When there is only one wildcard, the candidates are just the symbols of \(F\).  
	We can order them as \((f_1) \;\; f_1 \in F\).  
	Clearly, consecutive candidates differ in exactly one coordinate, since there is only one coordinate.
	
	\item \textbf{Recursive step (\(k>1\)).}  
	Suppose we already have a Gray-code ordering of all \((k-1)\)-tuples from \([|F|]^{k-1}\).  
	To construct an ordering of all \(k\)-tuples:
	\begin{enumerate}
		\item Traverse the \((k-1)\)-tuples in Gray-code order.
		\item For the first tuple, append the last coordinate \(f_k\) in the order \(f_1,f_2,\dots,f_{|F|}\).
		\item For the second tuple, append the last coordinate in reverse order \(f_{|F|}, f_{|F|-1},\dots,f_1\).
		\item Alternate between forward and reverse orders as you progress through the list of \((k-1)\)-tuples.
	\end{enumerate}
	This construction ensures that within each block of candidates, consecutive strings differ only in the last coordinate,
	and between consecutive blocks, the transition changes exactly one of the first \(k-1\) coordinates.  
	Therefore, overall, every pair of consecutive candidates differs in exactly one coordinate.
\end{itemize}


In this ordering, moving from one candidate string to the next amounts to changing the symbol in exactly one wildcard 
position. Therefore, in the LCS data structure, we update only a single symbol substitution at each step.  
The cost of moving between consecutive candidates is thus reduced to a single update of cost \(\BigONotation(\log^8 \lengthT)\).

For each generated candidate, we query the LCS data structure against \(\textstr\).  
If the LCS length equals \(\lengthP\), then the candidate occurs as a substring of \(\textstr\), and hence the original 
pattern \(\pattern\) admits a valid match.  


Since the number of candidates is at most \((\tfrac{\lengthT}{\tau})^k\), and each requires a single update and a query 
costing \(\BigONotation(\log^8 \lengthT)\), the total time complexity for this case is
\[
\BigONotation\!\left( \left(\tfrac{\lengthT}{\tau}\right)^k \cdot \log^8 \lengthT \right).
\]

\begin{example}
Suppose the pattern is
\[
P = \texttt{U ? V ? X},
\]
where the two wildcard positions are \(w_1=2\) and \(w_2=4\).  
Here \(U,V,X\) denote fixed substrings of the pattern that contain no wildcards (possibly empty).  
Let the set of frequent symbols be \(F=\{a,b,c\}\), so \(|F|=3\).  

Each concrete candidate pattern is obtained by choosing a pair \((f_1,f_2)\in F^2\), where \(f_1\) is substituted at 
position \(w_1\) and \(f_2\) at position \(w_2\).  
For instance, the pair \((a,c)\) yields the candidate \(\texttt{U a V c X}\).  

We generate all pairs in Gray-code order so that each consecutive pair differs in exactly one coordinate. 
One valid ordering is:
\[
(a,a)\;\to\;(a,b)\;\to\;(a,c)\;\to\;(b,c)\;\to\;(b,b)\;\to\;(b,a)\;\to\;(c,a)\;\to\;(c,b)\;\to\;(c,c).
\]

Mapping these pairs to candidates gives:
\[
\begin{array}{c|c|c}
	\text{pair }(f_1,f_2) & \text{changed coordinate} & \text{candidate string}\\ \hline
	(a,a) & - & \texttt{U a V a X}\\
	(a,b) & f_2 & \texttt{U a V b X}\\
	(a,c) & f_2 & \texttt{U a V c X}\\
	(b,c) & f_1 & \texttt{U b V c X}\\
	(b,b) & f_2 & \texttt{U b V b X}\\
	(b,a) & f_2 & \texttt{U b V a X}\\
	(c,a) & f_1 & \texttt{U c V a X}\\
	(c,b) & f_2 & \texttt{U c V b X}\\
	(c,c) & f_2 & \texttt{U c V c X}
\end{array}
\]

Since consecutive candidates differ in exactly one wildcard position, transitioning from one row to the next requires 
only a single-symbol update in the LCS data structure. Thus each step costs \(\BigONotation(\log^8 \lengthT)\).
\end{example}


==> src/our-results.tex <==
\section{Our Results}
\label{sec:our_results}

In this section, we present the key outcomes of our research on the dynamic pattern matching problem, focusing on variants with fixed and general wildcards. Our algorithms address the challenge of efficiently handling updates to both the pattern and text while maintaining high accuracy in match detection. We provide preprocessing and update/query time complexities that reflect trade-offs between computational cost and the number of wildcards or text length. Additionally, the algorithms offer probabilistic guarantees: matches are reported with probability 1 when they exist, and no match is reported with a probability approaching 1 when none exists, based on the choice of a sufficiently large prime modulus. The following table summarizes the results for each problem variant, showcasing the achieved complexities and their reliability.

\begin{table}[ht]
	\centering
	\caption{Summary of Results for Dynamic Pattern Matching Variants}
	\label{tab:results}
	\renewcommand{\cellalign}{tl} % align top-left in cells
	\setlength{\extrarowheight}{2pt} % extra space for readability
	\begin{tabularx}{\textwidth}{@{}lXlX@{}}
		\toprule
		Problem Variant & Preprocessing Time & Update/Query Time & Match Reporting Probability \\
		\midrule
		Dynamic pattern matching with fixed wildcards &
		\(\BigONotation(n \log^2 n)\) &
		\makecell[l]{%
			\(\BigONotation\Big(k\,n^{1 - \frac{1}{(\ln n)^\alpha}} \log n + n^{1 - \frac{1}{(\ln n)^\alpha}} \log n\)\\
			\(+ n^{\frac{k}{(\ln n)^\alpha}} \log^8 n + k^3 \log n \Big)\)%
		} &
		\makecell[l]{Match: 1 when exists \\ No match: \(1 - (1 - 1/n^{10})^{n-m+1}\)} \\
		\addlinespace
		Dynamic pattern matching with fixed wildcards (\(w\) non-wildcards) &
		- &
		\(\BigONotation(w + \log n)\) &
		\makecell[l]{Match: 1 when exists \\ No match: \(1 - (1 - 1/n^{10})^{n-m+1}\)} \\
		\addlinespace
		Dynamic pattern matching with fixed wildcards (\(m\)) &
		\(\BigONotation(m n)\) &
		\(\BigONotation(m + \log n)\) &
		\makecell[l]{Match: 1 when exists \\ No match: \(1 - (1 - 1/n^{10})^{n-m+1}\)} \\
		\addlinespace
		Dynamic pattern matching with wildcards &
		\(\displaystyle \BigONotation\Big((n/\tau + 1)^k \log^8 n + \tau k \log_2 n\Big)\) &
		- &
		\makecell[l]{Match: 1 when exists \\ No match: \(1 - (1 - 1/n^{10})^{n-m+1}\)} \\
		\addlinespace
		Dynamic pattern matching with wildcards (at most 2 non-wildcards) &
		\(\BigONotation(n^{1.8})\) &
		\(\BigONotation(n^{0.8} \log n)\) &
		Deterministic \\
		\bottomrule
	\end{tabularx}
\end{table}

==> src/phassmall.tex <==
\textbf{\(P\) contains a rare symbol:}
If the pattern \(\pattern\) contains a rare symbol \(c\) at some position \(i\) (i.e., \(\pattern_i = c\)), 
then any valid match in the text must align this occurrence of \(c\) with the same symbol in \(\textstr\). In other 
words, for a match to occur, we must have \(\textstr_j = c\) for some position \(j\) in \(\textstr\).  

Since \(c\) is rare, it appears at most \(\tau\) times in the initial text. Moreover, at most \(\tau\) additional 
occurrences can be introduced through change queries. Thus, the total number of positions where \(\textstr_j = c\) 
can never exceed \(2\tau\).  

To identify potential matches, we scan only these candidate positions \(j\) using the occurrence set \(\mathfrak{R}(c)\). For
each such \(j\), we verify whether \(\pattern\) matches the substring \(\textstr_{j-i+1 : j-i+m}\). This check is
performed via the procedure
\[
\texttt{is\_match}(\pattern, \textstr_{j-i+1 : j-i+m}),
\]
which, by Theorem~\ref{thm:is_match_hash_query}, confirms a match in \(\BigONotation(k \log \lengthT)\) time. Since there are at most \(\BigONotation(\tau)\) candidate positions, the total time required for this case is
\[
\BigONotation(\tau \cdot k \log \lengthT).
\]

\begin{figure}[t]
	\centering
	\scalebox{0.85}{
		\begin{tikzpicture}[
			box/.style={draw, thick, rounded corners, minimum size=0.6cm, font=\ttfamily},
			patternbox/.style={box, fill=blue!10, draw=blue!60},
			wildcardbox/.style={box, fill=yellow!20, draw=orange!60},
			textbox/.style={box, fill=green!10, draw=green!60},
			index/.style={font=\footnotesize, below, text=gray},
			matchrect/.style={draw=blue!80, thick, dashed, rounded corners},
			arrow/.style={-stealth, thick, red!80},
			nonwildmatch/.style={draw=red!80, very thick, rounded corners},
			background/.style={fill=gray!5, draw=gray!20, rounded corners}
			]
			
			% ==== Pattern ====
			\node[anchor=east] at (-0.5, 2) {\(\pattern =\)};
			\foreach \i/\char in {1/a, 2/v, 3/\texttt{?}, 4/b, 5/\texttt{?}, 6/c, 7/d, 8/e, 9/f} {
				\begin{scope}[shift={(\i,2)}]
					\ifnum\i=3 \node[wildcardbox] (p\i) {\char};
					\else \ifnum\i=5 \node[wildcardbox] (p\i) {\char};
					\else \node[patternbox] (p\i) {\char};
					\fi\fi
					\node[index] at (0,-0.4) {\i};
				\end{scope}
			}
			
			% ==== Text ====
			\node[anchor=east] at (-0.5, 0) {\(\textstr =\)};
			\foreach \i/\char in {1/x, 2/a, 3/v, 4/t, 5/b, 6/y, 7/c, 8/d, 9/e, 10/f, 11/z} {
				\begin{scope}[shift={(\i,0)}]
					\node[textbox] (t\i) {\char};
					\node[index] at (0,-0.4) {\i};
				\end{scope}
			}
			
			% ==== Matching rectangle ====
			\draw[matchrect] (1.55,-1) rectangle (10.45,1);
			
			% ==== Red box around consecutive 'av' in pattern and text ====
			\node[nonwildmatch, fit=(p1)(p2)] {}; % pattern 'a','v'
			\node[nonwildmatch, fit=(t2)(t3)] {}; % text 'a','v'
			
			% ==== Red box around 'cdef' in pattern and text ====
			\node[nonwildmatch, fit=(p6)(p9)] {}; % pattern c d e f
			\node[nonwildmatch, fit=(t7)(t10)] {}; % text c d e f
			
			% ==== Single non-wildcard match (b) ====
			\node[nonwildmatch,fit=(p4)] {}; 
			\node[nonwildmatch,fit=(t5)] {}; 
			
			% ==== Arrows from pattern to text ====
			\foreach \pi/\ti in {1/2, 2/3, 4/5, 6/7, 7/8, 8/9, 9/10} {
				\draw[arrow] (p\pi.south) -- (t\ti.north);
			}
			
			% ==== Background frame ====
			\begin{scope}[on background layer]
				\node[background, inner sep=5mm, fit=(current bounding box)] {};
			\end{scope}
			
		\end{tikzpicture}
	}
	\caption{Pattern: \(av?b?cdef\). Text: \(xavtbycdefz\). Red boxes show grouped consecutive non-wildcard matches: "av", "b", and "cdef".}
	\label{fig:rare-merged-fixed-styled}
\end{figure}


==> src/queries.tex <==
\section{Queries}
We define two types of queries in this section.\comment[id=ms]{Add affilication.t}
\comment[id=ms]{Move Queries to Preliminaries after we define our basic notations.}
\subsection{Hash Queries}
\comment[id=ms]{define the set of symbols.}
\comment[id=ms]{The definitions must be far more accurate. What is Hash function?  What is $S[l,r]$.}
Consider a string \( S \) and a hash function \( \hashFunc{\cdot} \), which is defined on \( S \) such that \( \hashFunc{S_{l:r}} \) can be computed using \( \hashFunc{S_{l:i}} \) and \( \hashFunc{S_{i+1:r}} \) in \( \BigONotation(1) \).  
The queries for this problem are as follows:
\begin{itemize}
	\item Update \( S_i \) to a new character.
	\item Compute \( \hashFunc{S_{l:r}} \).
\end{itemize}
We handle these queries in \( \BigONotation(\log_2 n) \) using a segment tree. 
\comment[id=ms]{either cite a paper or say how.}
\subsection{Existence Queries}
Consider a static vector \( A \). We need to process the following query:  
\[
\text{exist}(A_{l:r}, x)
\]
which determines whether the number \( x \) appears in the subvector (contiguous) \( A_{l:r} \).  
We answer this query in \( \BigONotation(\log_2 n) \) using a segment tree or a Fenwick tree.\comment[id=ms]{either cite a paper or say how.}


==> src/somewildcardmatchtosmall.tex <==
\noindent\textbf{Some wildcards match a rare symbol.}  
In this final case, we focus on matches where at least one wildcard in \(\pattern\) aligns with a rare symbol in 
\(\textstr\). Several important restrictions follow from the cases already considered.  
First, if a valid match did not involve any change in \(\textstr\), it would have been detected in 
Case~(ii), so here we may assume that the match uses at least one symbol that was introduced or modified by an update 
to \(\textstr\).  
Second, if every wildcard in \(\pattern\) aligned only with frequent symbols, then the situation would fall under 
Case~(iii).  
Finally, we can also rule out the possibility that \(\pattern\) itself contains rare symbols, since that was already 
treated in Case~(i).  
Thus, the only remaining possibility is that the match involves at least one rare symbol from \(\textstr\) that is 
aligned with a wildcard in \(\pattern\), and that this alignment necessarily occurs in a region of the text affected by 
an update.


We now formalize the notion of a \emph{candidate position}.  
A position \(\textstr_{i}\) in the text is called a candidate if it satisfies two conditions:
\begin{enumerate}
	\item \(\textstr_{i}\) is a rare symbol.  
	\item There exists a substring interval \(\textstr_{j:j+\lengthP-1}\) of length \(\lengthP\) that contains 
	position \(i\), includes at least one position that has been modified by an update query, and contains at most \(k\) 
	rare symbols in total (including \(\textstr_{i}\) itself).
\end{enumerate}
 

We bound the number of such candidates. Consider a changed position \(p\) in \(\textstr\). Any valid match involving 
\(p\) can only include rare symbols that are close to \(p\), because each match interval of length \(\lengthP\) may 
contain at most \(k\) rare symbols in total. Thus, for each side of \(p\), at most the \(k\) nearest rare symbols can 
qualify as candidates. To see this, suppose we look farther than the \(k\)-th nearest rare symbol on one side. Then the 
interval covering both that symbol and \(p\) would necessarily contain at least \(k+1\) rare symbols, violating the 
requirement of condition (b). Therefore, each changed position contributes at most \(2k\) candidates: \(k\) to the left 
and \(k\) to the right.  
Since there are at most \(\tau\) changed positions in total, the total number of candidate positions is bounded by
$
\BigONotation(\tau \cdot k).
$


For each candidate position \(i\), we must test all possible alignments of \(\textstr_{i}\) with the wildcards of 
\(\pattern\). Specifically, \(i\) may correspond to the first wildcard at position \(w_1\), the second at \(w_2\), and so 
on, up to the \(k\)-th wildcard at \(w_k\). Thus, there are at most \(k\) possible alignments for each candidate.  

Consider a particular alignment where \(\textstr_{i}\) is matched to the wildcard at position \(w_\ell\). In this case, the 
relevant substring of the text is \(\textstr_{i - w_\ell + 1:i - w_\ell + \lengthP}\), which is the length-\(\lengthP\) 
interval that aligns \(\textstr_{i}\) with \(w_\ell\). To check this substring efficiently, we compute its modified hash 
\(\hashPrimeFunc{\cdot}\), which ignores wildcard positions. This is done by splitting the substring into its \(k+1\) 
non-wildcard segments, evaluating the hash \(\hashFunc{\cdot}\) of each segment in \(\BigONotation(1)\) time, and concatenating them using Lemma~\ref{lem:concat_hash_efficiency}. The total cost per alignment is 
therefore \(\BigONotation(k)\).  



Once the hashes \(\hashPrimeFunc{\cdot}\) for all candidate substrings are computed, we must store them in a data 
structure that allows us to efficiently check whether the current pattern hash \(\hashPrimeFunc{\pattern}\) appears among 
them. For this purpose we use a balanced binary search tree, which supports 
three key operations in \(\BigONotation(\log \lengthT)\) time each:  
\begin{itemize}
	\item \emph{Insertion:} add a new hash value corresponding to a candidate alignment,  
	\item \emph{Deletion:} remove an outdated hash value when the underlying text substring changes,  
	\item \emph{Membership query:} check whether a given hash value (e.g., \(\hashPrimeFunc{\pattern}\)) exists in the tree.  
\end{itemize}

We now analyze the number of hash values stored.  There are at most \(\BigONotation(\tau \cdot k)\) candidate positions overall. Each candidate position may align with any of the \(k\) wildcards of the pattern, giving up to \(k\) alignments.  Thus, the total number of candidate alignments is bounded by \(\BigONotation(\tau \cdot k^2)\).  
For each such alignment we must compute \(\hashPrimeFunc{\cdot}\). This takes \(\BigONotation(k)\) time (to combine the 
\(k{+}1\) non-wildcard segments) and then requires \(\BigONotation(\log \lengthT)\) time to insert into the balanced tree. Hence, 
the cost per alignment is \(\BigONotation(k + \log \lengthT)\). Multiplying by the total number of alignments, the total cost of 
initializing and populating the tree is
\[
\BigONotation\!\big(\tau \cdot k^2 \cdot (k + \log \lengthT)\big).
\]

This initialization is performed once per rebuilding phase, which occurs after every \(\tau\) queries. Therefore, the 
per-query amortized cost of maintaining this data structure is
\[
\BigONotation(k^3 + k^2 \log \lengthT).
\]

When the pattern \(\pattern\) changes, the update is straightforward.  
We recompute its modified hash \(\hashPrimeFunc{\pattern}\) in \(\BigONotation(k)\) time by combining the 
\(k{+}1\) non-wildcard segments.  
We then query the balanced search tree to check whether this hash value appears among the stored substring hashes of 
\(\textstr\).  
The membership query takes \(\BigONotation(\log \lengthT)\) time.  
If the hash is found, we conclude that \(\pattern\) matches a substring of \(\textstr\); otherwise, no match exists.  

When the text \(\textstr\) is updated at some position \(p\), the situation is more involved.  
A modification at \(p\) can potentially affect only those candidate substrings that contain \(p\).  
As shown earlier, this means at most the \(k\) nearest rare symbols to the left of \(p\) and the \(k\) nearest to the right 
need to be reconsidered, giving \(\BigONotation(k)\) candidates in total.  

For each affected candidate \(i\), we must update the hashes corresponding to all of its \(k\) possible alignments 
(with the \(k\) wildcards of \(\pattern\)).  
This requires three steps:
\begin{enumerate}
	\item \emph{Deletion:} remove the old hash values for the \(k\) alignments from the balanced tree.  
	Each deletion costs \(\BigONotation(\log \lengthT)\), for a total of \(\BigONotation(k \log \lengthT)\).  
	\item \emph{Recomputation:} compute the new hash values for the same \(k\) alignments.  
	Each recomputation takes \(\BigONotation(k)\) time, giving a total of \(\BigONotation(k^2)\).  
	\item \emph{Insertion:} insert the updated hashes into the balanced tree.  
	Each insertion also costs \(\BigONotation(\log \lengthT)\), so again \(\BigONotation(k \log \lengthT)\) in total.  
\end{enumerate}

Thus, the total cost of processing one candidate is 
$\BigONotation(k^2 + k \log \lengthT).$   
Since there are \(\BigONotation(k)\) candidates per text update, the overall update cost is
\[
\BigONotation(k^3 + k^2 \log \lengthT).
\]

In summary, pattern updates can be processed in \(\BigONotation(k + \log \lengthT)\) time, while text updates require 
\(\BigONotation(k^3 + k^2 \log \lengthT)\) time.  

\begin{figure}[t]
	\centering
	\scalebox{0.7}{
		\begin{tikzpicture}[
			box/.style={minimum size=0.9cm, draw=gray!50, thick, fill=white, rounded corners, font=\ttfamily\small, align=center},
			rarecolor/.style={box, fill=blue!40, draw=blue!80, very thick},
			rareplus/.style={box, fill=yellow!80, draw=yellow!70!black, very thick},
			changecolor/.style={box, fill=pink!70, draw=red!70, very thick},
			labeltext/.style={font=\scriptsize, text=black},
			background/.style={fill=gray!5, draw=gray!20, rounded corners},
			]
			
			% سه نقطه اول
			\node at (1,0) {\(\dots\)};
			\node[rareplus] at (2,0) {};
			\node[box] at (3,0) {};
			\node[rarecolor] at (4,0) {};
			\node[rarecolor] at (5,0) {};
			\node at (6,0) {\(\dots\)};
			\node[box] at (7,0) {};
			\node[rarecolor] at (8,0) {};
			\node[box] at (9,0) {};
			\node[changecolor] at (10,0) {};
			\node[labeltext, above] at (10,0.5) {changed position};
			\node[box] at (11,0) {};
			\node[rarecolor] at (12,0) {};
			\node at (13,0) {\(\dots\)};
			\node[box] at (14,0) {};
			\node[rarecolor] at (15,0) {};
			\node[box] at (16,0) {};
			\node[rarecolor] at (17,0) {};
			\node[rareplus] at (18,0) {};
			\node[box] at (19,0) {};
			\node at (20,0) {\(\dots\)};
			
			% label T چپ
			\node[align=center] at (0,0) {\(\textstr =\)};
			
			% legend بالا سمت راست
			\node[draw, fill=white, rounded corners, inner sep=4pt, above left, xshift=-0.5cm, yshift=0.8cm] 
			at (current bounding box.north east) {
				\begin{tabular}{@{}ll@{}}
					\raisebox{-.4ex}{\tikz{\node[rarecolor] {};}} & rare symbol \\
					\raisebox{-.4ex}{\tikz{\node[rareplus] {};}} & \(k{+}1\)-th rare symbol \\
				\end{tabular}
			};
			
			
			
			% قاب پس زمینه کلی
			\begin{scope}[on background layer]
				\node[background, inner sep=6mm, fit=(current bounding box)] {};
			\end{scope}
			
		\end{tikzpicture}
	}
	\caption{Only the first \(k\) rare symbols to the left and right of the change position are examined. The \(k{+}1\)th rares are not used.}
	\label{fig:rare-selection-final}
\end{figure}




